GPU coprocessors as a service for deep learning inference in high energy physics

In the next decade, the demands for computing in large scientific experiments are expected to grow tremendously. During the same time period, CPU performance increases will be limited. At the CERN Large Hadron Collider (LHC), these two issues will confront one another as the collider is upgraded for high luminosity running. Alternative processors such as graphics processing units (GPUs) can resolve this confrontation provided that algorithms can be sufficiently accelerated. In many cases, algorithmic speedups are found to be largest through the adoption of deep learning algorithms. We present a comprehensive exploration of the use of GPU-based hardware acceleration for deep learning inference within the data reconstruction workflow of high energy physics. We present several realistic examples and discuss a strategy for the seamless integration of coprocessors so that the LHC can maintain, if not exceed, its current performance throughout its running.

==> HcalAlgo.tex <==
The simplest algorithm designed for these studies is FACILE, a deep neural network composed of 2,000 parameters and five fully-connected dense layers. This algorithm was trained on simulated LHC collision data to reconstruct the energy deposited by particles in the Hadron Calorimeter (HCAL) subdetector, a key component of LHC all-purpose detectors. The HCAL is the first subdetector we apply reconstruction via deep learning as a service for two reasons. 

Firstly, good resolution in the HCAL is essential for sensitive measurements in particle physics, such as events with a Higgs boson decaying to quarks. In studies comparing the resolution obtained on objects from FACILE with objects reconstructed with the nominal reconstruction algorithm, we find that FACILE offers improved resolution over the nominal HCAL algorithm. This effect is stronger at lower energy scales because FACILE is sensitive to additional collisions occuring within the time region of interest. Secondly, the nominal HCAL reconstruction algorithm consumes about 60 ms of CPU time in online reconstruction, accounting for 15\% of the online computing budget. FACILE offers improved computing performance when operated as a service by reducing the CPU time to 7 ms. This is because the remote time (including 2 ms of GPU inference time) is eliminated by the asynchronous, non-blocking call for external work utilized in SONIC. 

In this study, we deploy FACILE as a service in both online and offline reconstruction. The online test is an emulation of the partial-reconstruction consisting of 20,000 CPUs at CERN. The offline test is XXX. 

==> cost.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\cline{1-9} 
\textbf{Algorithm} &  \textbf{\textit{Inf/GPUs}} & \textbf{\textit{GPUs/Offline}} & \textbf{\textit{Cost/day}} & \textbf{\textit{Egress Throughput}}  & \textbf{\textit{Egress}} & \textbf{\textit{Throughput}}  & \textbf{\textit{Load balance}} & Total Cost  \\
 & & & Cost & [Gbit/s] & Cost & [Gbit/s] & [Gbit/s] & 1/day \\
\hline
FACILE     & 500  & 10 & \$590  & 2.56                & \$18k & 39\unit{Gb/s}  & \$26.5\,k/day & \$44.8 \,k/day\\
DeepCalo   & 680  & 8  & \$470  & 1.7$\times 10^{-3}$ & \$1.2 & 2.4\unit{Gb/s} & \$1.7\,k/day  & \$2.1 k/day\\
DeepCalo*  & 9800 & 1  & \$59   & 1.7$\times 10^{-3}$ & \$2.2 & 2.4\unit{Gb/s} & \$1.7\,k/day  & \$1.7 k/day \\ 
ResNet-50   & 25   & 20 & \$1180 & 1.6$\times 10^{-5}$ & \$0.1 & 24\unit{Gb/s}  & \$16.6\,k/day & \$17.8 k/day\\ 
\hline
\end{tabular}
\end{center}
\label{tab:algosummary}
\end{table}


==> networkParameters.tex <==
\begin{table}
\begin{center}
\caption{Summary of the timing metrics for each model, including CPU latency (X) (as measured on a single-core AMD Gen 3 Class Opteron @ 2.0 GHz for FACILE and ResNet50, Intel(R) Xeon(R) CPU E5-2698 v4 @ 2.20GHz for DeepCalo), GPU latency (Y), and SONIC client overhead time (S). The asterisk (*) indicates a comparison to the nominal Hadron Calorimeter reconstruction algorithm operating on CPU.}

\begin{tabular}{|l|c|c|c|}
\cline{1-4} 
\textbf{Algorithm} &  
\textbf{\textit{CPU latency (X)}} &
\textbf{\textit{GPU latency (Y)}} & 
\textbf{\textit{SONIC time (S)}} \\
& [ms] & [ms] & [ms] \\
\hline
FACILE     & 60* & 2 & 1 \\
DeepCalo   & 75 & 1.5  & 0.01 \\
ResNet50   & 8000 & 40  & 0.01 \\
\hline
\end{tabular}
\end{center}
\label{tab:algotimes}
\end{table}
